Multimedia Services Placement Algorithm for Cloud-Fog Hierarchical Environments

With the rapid development of mobile communication, multimedia services have experienced explosive growth in the last few years. The high quantity of mobile users, both consuming and producing these services to and from the Cloud Computing (CC), can outpace the available bandwidth capacity. Fog Computing (FG) presents itself as a solution to improve on this and other issues. With a reduction in network latency, real-time applications benefit from improved response time and greater overall user experience. Taking this into account, the main goal of this work is threefold. Firstly, it is proposed a method to build an environment based on Cloud-Fog Computing (CFC). Secondly, it is designed two models based on Autoregressive Integrated Moving Average (ARIMA) and Long Short-Term Memory (LSTM). The goal is to predict demand and reserve the nodes' storage capacity to improve the positioning of multimedia services. Later, an algorithm for the multimedia service placement problem which is aware of data traffic prediction is proposed. The goal is to select the minimum number of nodes, considering their hardware capacities for providing multimedia services in such a way that the latency for servicing all the demands is minimized. An evaluation with actual data showed that the proposed algorithm selects the nodes closer to the user to meet their demands. This improves the services delivered to end-users and enhances the deployed network to mitigate provider costs. Moreover, reduce the demand to Cloud allowing turning off servers in the data center not to waste energy

==> biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/fillipe}}]{Fillipe Santos}
is a master's degree student at the Institute of Computer Science at State University of Campinas (UNICAMP).
He received his bachelor’s degree in Computer Science from the Federal University of Alagoas, Brazil, in 2017.
His research interests include vehicular ad hoc networks. 
Also, he has published some papers in the area of Autonomous Aerial Vehicles and Fog Computing.
\end{IEEEbiography}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/alla}}]{Andre L. L. Aquino}
%(alla@laccan.ufal.br) 
is a Professor at Federal
University of Alagoas, Brazil. He received his Ph.D. in Computer Science from the Federal University of Minas Gerais, Brazil, in 2008. His research interests include data reduction, distributed algorithms, wireless ad hoc and sensor networks, mobile and pervasive computing. In addition, he has published several papers in the area of wireless sensor networks.
\end{IEEEbiography}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/edmundo}}]{Edmundo R. M. Madeira} 
%(edmundo@ic.unicamp.br) Edmundo R. M. Madeira 
received the PhD
degree in electrical engineering from University of
Campinas (UNICAMP), in 1991. He is a full professor with the University of Campinas, Brazil. He
has published more than 150 papers in national
and international conferences and journals. He
was the general chair of the 7th Latin American
Network Operation and Management Symposium (LANOMS’11), and a TPC co-chair of the
IEEE LatinCloud’12. He also is a TPC co-chair of
the 15th IFIP/IEEE International Symposium on
Integrated Network Management (IM 2017). He is a member of the editorial board of the Journal of Network and Systems Management
(JNSM), Springer. His research interests include network management,
future Internet, and cloud computing. He is a member of the IEEE.
\end{IEEEbiography}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/raquel.pdf}}]{Raquel S Cabral}
%(raquel.cabral@arapiraca.ufal.br) 
is a Professor at Federal
University of Alagoas, Brazil. He received his Ph.D. in Electrical Engineering from the Federal University of Minas Gerais, Brazil, in 2013.
His research interests include complex network and optimization.
In addition, he has published papers in the area of wireless
sensor networks and complex networks and statistics.
\end{IEEEbiography}

